CPL: A Core Language for Cloud Computing -- Technical Report

Running distributed applications in the cloud involves deployment. That is, distribution and configuration of application services and middleware infrastructure. The considerable complexity of these tasks resulted in the emergence of declarative JSON-based domain-specific deployment languages to develop deployment programs. However, existing deployment programs unsafely compose artifacts written in different languages, leading to bugs that are hard to detect before run time. Furthermore, deployment languages do not provide extension points for custom implementations of existing cloud services such as application-specific load balancing policies. To address these shortcomings, we propose CPL (Cloud Platform Language), a statically-typed core language for programming both distributed applications as well as their deployment on a cloud platform. In CPL, application services and deployment programs interact through statically typed, extensible interfaces, and an application can trigger further deployment at run time. We provide a formal semantics of CPL and demonstrate that it enables type-safe, composable and extensible libraries of service combinators, such as load balancing and fault tolerance.

==> actors.tex <==

\subsection{Fault Tolerance and Hierarchical Supervision}
\label{sec:case-study:-hier}


Fault tolerant actor systems like Akka\footnote{\url{http://akka.io}}
and Erlang OTP~\cite{Armstrong:1996:CPE:229883} are organized in tree
structures, where
parent actors actively monitor their children to detect crashes and take appropriate measures, such as restarting
failed children or in turn notifying the parent actor. Also, children proactively notify the parent of any exception. 

In the case study,
we abstract over actors and model \emph{component} servers which are monitored
by \emph{supervisor} servers, i.e., a supervisor monitors exactly one component server and has a reference
to multiple child supervisors and a reference to its parent supervisor. 
We define a reusable generic combinator which can establish such a supervision tree. The interface for component servers 
is the following:
{\small
\begin{align*}
\Type{TComp} := \Tsrv{(& \id{suspend}\tpe < <> >, \id{resume}\tpe < <>  >, \id{restart}\tpe < <> >, \\ 
                      & \!\!\!\!\!\!\!\id{supervisor}\tpe < \Tsrvinst{\Tsrv{( \id{onError}\tpe<\Type{TErr}> ) }} >  )}.
\end{align*}
}%
That is, a component at least offers services for pausing, resuming and restarting as well as 
a state service $\id{supervisor}$ which holds a reference to its monitoring supervisor. The supervisor
must provide an $\id{onError}$ service accepting an error description of type $\Type{TErr}$, which we leave underspecified.
Components notify an exception the supervisor via the $\id{onError}$ service.

A supervisor must implement the interface of the child type in case it is also supervised.
\begin{align*}
\Type{TChild} := \Tsrv{(&\id{suspend}\tpe < <> >, \id{resume}\tpe < <> >, \\
& \id{restart}\tpe < <> >, \id{stop}\tpe < <> >)},
\end{align*}
The full interface of a supervisor adds more services for its role as a parent:
%
\\[1ex]
\noindent$
\begin{array}{ll}
 \multicolumn{2}{l}{\Type{TSupervisor} := \Type{TChild}\cup\Tsrv{(}} \\
 & \!\!\!\! \id{children}\tpe <\Type{List}[\Tsrvinst{\Type{TChild}}]>,\  \id{addChild}\tpe <\Tsrvinst{\Type{TChild}}>, \\
 & \!\!\!\! \id{onError}\tpe <\Type{TErr}>,\ \id{childError}\tpe <\Tsrvinst{\Type{TChild}}, \Type{TErr}>) .
\end{array}
$\\[1ex]
That is, a supervisor has the server template of a child and it maintains a list of child supervisors in the
state service $\id{children}$, where the service $\id{addChild}$ inserts new children into the list.
As motivated before, it has the callback service $\id{onError}$ for receiving error notifications
of the monitored component. The additional service \id{childError} handles errors reported
by the child supervisors and crashes detected by the parent.

            
Supervisors react to children errors according to \emph{Supervision strategies}. 
In the \emph{OneForOne} strategy if one child fails, only the failed child is restarted. In the \emph{AllForOne} strategy
every child must be restarted, not only the failed one.
For brevity, we show only the OneForOne strategy. AllForOne just
applies the same actions to all children.

Exception handling is modeled by a function\footnote{Recall our function encoding from section~\ref{sec:derived-syntax}.}
$$
\Type{TDecider} := \Type{TErr} \to \Type{TDirective},
$$
where $\Type{TDirective}$ is a church encoded enumeration type for supervisor actions:
$$
\Type{TDirective} := \Type{Escalate} \mid \Type{Stop} \mid \Type{Resume} \mid \Type{Restart}.
$$
When a monitored component encounters an exception
and notifies its supervisor via the $\id{onError}$ service, the supervision protocol (1) suspends the component,
(2) recursively suspends each child supervisor, i.e., the entire subtree with the supervisor as root is suspended and (3) suspends itself and notifies its parent.

The parent invokes its \Type{TDecider} with the current error value, which yields one of the 
four choices for \Type{TDirective}. \Type{Escalate} -- 
recursively suspend its children and itself and propagate the exception to the next parent.
\Type{Stop} -- the suspended child subtree is recursively terminated and removed. \Type{Resume} -- the child subtree is recursively resumed, preserving
the internal state of the monitored components. \Type{Restart} --
the failed child will create a new instance of its monitored component, recursively restart its own
children and resume operation.

Invoking
the \id{OneForOne} factory instantiates a new supervisor node to monitor a component:
{\small
  \begin{align*}
\Tsrvinst{& \Tsrv{ \id{make}\tpe \\
          & \!\!\!\!\!\! (\Tsrvinst{\Type{TSupervisor}}, \Type{TComp}, \Type{TDecider}) \to \Tsrvinst{\Type{TSuperVisor}}}}.
  \end{align*}
}%
Constructing a supervisor ($\id{make}$) requires the address of the parent\footnote{We assume the existence of a special root supervisor node, which we leave underspecified for brevity.},
the server template of the component to monitor and a decider function for the supervision strategy.

In the study we use the snapshot and replacement primitives for the implementation of suspend/resume. A supervisor node suspends itself and the monitored component instance by replacing and storing its own server image.
To this end, it invokes a factory $$\svc{\id{Suspended}}{\id{become}}<\<this>, \<snap> \<this>, \id{comp}, \id{cs}>, $$
which produces and manages a \emph{different behavior} for the supervisor. The factory replaces via the $\<repl>\!\!$ syntactic form the 
supervisor image by a stub implementing only resume, restart and stop. 
%
For a resume operation 
the suspended supervisor just has to invoke $\<repl>\!\!$ again
with the previously stored images to restore itself and the monitored component and recursively do so for the children.
%
Restarting is similar. In Akka, a restart of an actor entails resetting internal state,
but preserving unprocessed messages. We model this in the supervisor: Before restarting the component
the supervisor filters the buffer of the component's server image, leaving only unprocessed messages.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> implementation.tex <==

\section{Implementation}
\label{sec:implementation}

We have implemented the small-step reduction semantics and the type system of
\lang{} in PLT Redex~\cite{FelleisenFF09Redex}. Experimentation
with this implementation guided our design. In addition, we have implemented the type system and a \emph{big-step}
implementation of our semantics in Scala\footnote{The source code of the PLT
  Redex and Scala implementations and of all case studies is available online:
  \implementation.}, providing concurrent, thread-based execution. 
All the examples from this paper are executable in our implementation.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "report"
%%% End: 

